Inferring incompressible two-phase flow fields from the interface motion using physics-informed neural networks

In this work, physics-informed neural networks are applied to incompressible two-phase flow problems. We investigate the forward problem, where the governing equations are solved from initial and boundary conditions, as well as the inverse problem, where continuous velocity and pressure fields are inferred from scattered-time data on the interface position. We employ a volume of fluid approach, i.e. the auxiliary variable here is the volume fraction of the fluids within each phase. For the forward problem, we solve the two-phase Couette and Poiseuille flow. For the inverse problem, three classical test cases for two-phase modeling are investigated: (i) drop in a shear flow, (ii) oscillating drop and (iii) rising bubble. Data of the interface position over time is generated by numerical simulation. An effective way to distribute spatial training points to fit the interface, i.e. the volume fraction field, and the residual points is proposed. Furthermore, we show that appropriate weighting of losses associated with the residual of the partial differential equations is crucial for successful training. The benefit of using adaptive activation functions is evaluated for both the forward and inverse problem.

==> sections/highlights.tex <==
\section*{Highlights}

\begin{itemize}
    \item We extend the previous work on physics-informed neural networks to two-phase flows using a Volume-of-fluid approach and infer flow fields from scattered-time data of the interface position
    \item An effective way to distribute the training points used to fit the interface, i.e. the volume fraction field, and the residual points is proposed
    \item We give insight into the proper choice of hyper-parameters of the neural network and the training process
    \item The use of global and local adaptive activation functions is evaluated for more complex cases that they have been applied to so far
\end{itemize}
